Unsupervised Vehicle Counting via Multiple Camera Domain Adaptation

Monitoring vehicle flows in cities is crucial to improve the urban environment and quality of life of citizens. Images are the best sensing modality to perceive and assess the flow of vehicles in large areas. Current technologies for vehicle counting in images hinge on large quantities of annotated data, preventing their scalability to city-scale as new cameras are added to the system. This is a recurrent problem when dealing with physical systems and a key research area in Machine Learning and AI. We propose and discuss a new methodology to design image-based vehicle density estimators with few labeled data via multiple camera domain adaptations.

==> draftJP.tex <==
In  every  domain  of  life  and  society,  real-world  data  gains  pull  for  both  a  more  informed decision  making  and  citizenship. Serving this purpose, Artificial Intelligence  systems are front runners by their capacity to process huge amount of data and make decisions in complex scenarios where humans are at the epicentre. Compelling examples are city mobility, pollution monitoring or infrastructure management where decision-makers require precise measurements about how many entities of a certain class are present in a huge physical area (ex: bicycles, cars, people). Images obtained from cameras are signals that can cover such a dimension and simultaneously convey the "semantics" attached to those entities (objects ?). In this paper we will describe and discuss a methodology that computes the number of vehicles in a large scale scenario such as a city from images captured by a network of city cameras. We focus on vehicles because of its impact in the key scenarios described above, but the approach is general for any other "object".


 In particular, environmental monitoring is one application that could benefit from the assistance of AI systems in reducing air pollution in large and complex systems, such as modern cities, and improving our quality of life. To this end, this paper proposes an AI system that focuses on one of the most significant contributors to air pollution in urban areas -- traffic~\cite{zhang2013air}. Monitoring the traffic from surveillance cameras, namely by counting the number of vehicles circulating, is a crucial step towards better traffic flow management in cities~\cite{shirani2009store}, with a direct impact on air quality and on the economic growth and development of countries \cite{shafiei2018calibration}. 

%Nowadays, traffic congestion is continuously increasing and significantly hampering the economic growth and development of countries \cite{shafiei2018calibration}. Furthermore, traffic congestion increases vehicle emissions and degrades ambient air quality, and recent studies have shown excess morbidity and mortality for drivers, commuters, and individuals living near significant roadway \cite{zhang2013air}. Hence, the development of Intelligent Transportation Systems (ITS) able to predict traffic congestion and, in general, manage flow analysis have become of strategic importance.

%On the other hand, almost all modern cities are equipped with hundreds of smart surveillance cameras that also offer an incredible instrument for traffic density estimation. Unlike different types of sensors employed to collect traffic measurements, such as infrared captors, radars counters, and magnetic loops \cite{wei2013camera, saponara2017radar, ali2011multiple}, smart cameras are cheaper and more flexible. Perhaps most importantly, although the training phase of the CNNs is usually highly demanding in terms of computation, the inference phase can be exploited using less sophisticated hardware resources, e.g., directly onboard smart cameras, with a resulting high scalability. 
